A Modular Approach to Metatheoretic Reasoning for Extensible Languages

This paper concerns the development of metatheory for extensible languages. It uses as its starting point a view that programming languages tailored to specific application domains are to be constructed by composing components from an open library of independently-developed extensions to a host language. In the elaboration of this perspective, static analyses (such as typing) and dynamic semantics (such as evaluation) are described via relations whose specifications are distributed across the host language and extensions and are given in a rule-based fashion. Metatheoretic properties, which ensure that static analyses accurately gauge runtime behavior, are represented in this context by formulas over such relations. These properties may be fundamental to the language, introduced by the host language, or they may pertain to analyses introduced by individual extensions. We expose the problem of modular metatheory, i.e., the notion that proofs of relevant properties can be constructed by reasoning independently within each component in the library. To solve this problem, we propose the twin ideas of decomposing proofs around language fragments and of reasoning generically about extensions based on broad, a priori constraints imposed on their behavior. We establish the soundness of these styles of reasoning by showing how complete proofs of the properties can be automatically constructed for any language obtained by composing the independent parts. Mathematical precision is given to our discussions by framing them within a logic that encodes inductive rule-based specifications via least fixed-point definitions. We also sketch the structure of a practical system for metatheoretic reasoning for extensible languages based on the ideas developed.

==> ordering.tex <==
\section{Property Orders}
\label{sec:ordering}

In the preceding sections we have shown how we prove individual
properties will hold for the composed language based on modular proofs
written for them.  However, in the end, we are not interested in
whether individual properties hold, but in whether all properties
introduced by the host language and each extension included in a composed language will hold
based on the modular proofs written for them.

The host language and each extension has an associated order of
properties $\propset{}$ and an associated set of modular proofs
$\proofset{}$.  There is
a bijective mapping between the modular proofs
in $\proofset{}$ and the properties in the property order $\propset{}$
for the host language and each extension
(\ie{} each modular proof $\rho\in\proofset{}$ uniquely maps
to a property $P\in\propset{}$).
%
The properties are proven in the order in which they appear in
$\propset{}$, and this also determines which properties may be used as
lemmas in proving other properties.  Specifically, in proving the
properties in a property order $\propOrder{P_1,\ldots,P_m}$,
$\oneTo{P}{i-1}$ may be used as lemmas in a modular proof of $P_i$.

The property order given by the host language must be a subsequence of
each extension's order, with the extension adding new properties
anywhere in the host's order:  at the beginning, between two
preexisting properties, or at the end.
%
For example,
suppose the host language $H$ introduces three properties, $P^H_1$,
$P^H_2$, and $P^H_3$ and extension $A$ introduces a single new
property, $P^A_1$, and places it between $P^H_1$ and $P^H_2$.  Then
extension $A$'s property order $\propset{A}$ is
$\propOrder{P^H_1, P^A_1, P^H_2, P^H_3}$, leaving $\propset{H}$ as a
subsequence.  In modularly proving
$P^A_1$, extension $A$ may use $P^H_1$ as a lemma, and in fulfilling its proof
obligations for $P^H_2$ and $P^H_3$ it may use $P^A_1$ as a lemma.

In composing property orders, we must maintain the relative ordering
of properties from the host language and each extension so the same
lemmas will be available in the setting of the composition as in the
limited setting in which the modular proofs were written.
\begin{definition}[Property order composition] \label{def:prop-order-comp}
  Let $H$ be the host language and $E_1, \ldots, E_n$ be extensions in
  a language library.
  %
  Let $\propset{H}$ be the property order for $H$ and $\propset{E_i}$
  be the property order for extension $E_i$, $1 \leq i \leq n$.
  %
  The property order composition, written
  $\propComp{\propset{H}}{\propsetN{E}{n}}$, is an order of properties
  such that
  %
  each property order in
  $\setize{\propset{H},\propset{E_1},\ldots,\propset{E_n}}$
  is a subsequence of $\propComp{\propset{H}}{\propsetN{E}{n}}$.
\end{definition}
Because each extension's order contains the host language's order as a
subsequence, such a composition must exist.  In particular, we can
build a composition by concatenating the sub-orders of extension
properties occurring between two properties from the host language.
%
Building on our earlier property order example,
suppose a second extension $B$ has the property order
$\propOrder{P^H_1, P^B_1, P^B_2, P^H_2, P^H_3, P^B_3}$.  Since both
$\propOrder{P^A_1}$ and $\propOrder{P^B_1, P^B_2}$ occur between the
host language's properties $P^H_1$ and $P^H_2$, we concatenate them to
form a composition $\propComp{\propset{H}}{\setize{\propset{A},
    \propset{B}}} = \propOrder{P^H_1, P^A_1, P^B_1, P^B_2, P^H_2,
  P^H_3, P^B_3}$.  This composition has each composed order as a subsequence,
making it valid.

We also combine the modular proofs given by the host language and
each extension to form full proofs of all the properties.  The
bijective mapping between modular proofs and properties in
each \proofset{M} and \propset{M} will allow us to select the correct
modular proof for building the full proof of each property.

\begin{definition}[Full proof composition] \label{def:all-proof-comp}
  Let $H$ be the host language and let $E_1, \ldots, E_n$ be extensions
  in a language library.
  %
  Let $\proofset{H}$ be the set of modular proofs given by $H$ and
  $\proofset{E_i}$ be the set of modular proofs given by extension
  $E_i$, $1 \leq i \leq n$.
  %
  Let $\propset{H}$ be the order of properties given by $H$ and
  $\propset{E_i}$ be the order of properties given by extension $E_i$,
  $1 \leq i \leq n$.
  %
  Then the proof composition
  $\allProofComp{\proofset{H}}{\proofsetN{E}{n}}$ is the set of full
  proofs for each property in
  $\propComp{\propset{H}}{\propsetN{E}{n}}$.  Consider property $P$ in
  the composed properties:
  \begin{itemize}
  \item If $P$ is introduced by the host language ($P\in\propset{H}$),
    we add the proof given by \refdef{proof-comp} built from the
    modular proofs of $P$ in
    $\proofset{H},\proofset{E_1},\ldots,\proofset{E_n}$ to the full
    proof set.
  \item If $P = \forallx{\overline{x}}{R(\overline{t}) \imp F}$ is
    introduced by extension $E_i$ ($P\in\propset{E_i}$ and
    $P\notin\propset{H}$), we have a modular proof in $\proofset{E_i}$.
    We consider whether $R \in \relset{E_i}$
    or $R \in \relset{H}$:
    \begin{itemize}
    \item If $R \in \relset{E_i}$, we add the proof that is
      constructed based on \refthm{full-proof-ext} to the full proof set.
    \item If $R \in \relset{H}$, we add the proof that is constructed
      based on \refthm{full-proof-host} to the full proof set.
    \end{itemize}
  \end{itemize}
\end{definition}

Each property in the full proof composition has a valid proof in the
composed proof set.
\begin{thm} \label{thm:orderComp}
  Let $H$ be the host language and $E_1,\ldots, E_n$ be extensions in a
  language library.
  %
  Let $\propset{H}$ be the property order given by the host language
  and $\propset{E_1},\ldots,\propset{E_n}$ be the property orders given
  by the extensions.
  %
  Let $\proofset{H}$ be the set of modular proofs given by the host
  language and $\proofset{E_1},\ldots,\proofset{E_n}$ be the sets of
  modular proofs given by the extensions.
  %
  Assume each property in $\propset{M}$ has a corresponding valid
  modular proof in $\proofset{M}$, for $M\in\setize{H,E_1,\ldots, E_n}$.
  %
  Then $\allProofComp{\proofset{H}}{\proofsetN{E}{n}}$ contains a
  valid full proof for each property in
  $\propComp{\propset{H}}{\propsetN{E}{n}}$ for the language
  $\langComp{H}{\oneTo{E}{n}}$.
\end{thm}
\begin{proof}
  We start by noting that, for each property $P$ in the composed
  order, the modular proofs for it were written possibly using earlier
  properties as lemmas.  \refdef{prop-order-comp}, defining property
  order composition, ensures each lemma will still be an earlier
  property in the composed order, so uses of lemmas are still valid in
  the composition.
  %
  If $P$ was introduced by the host language, \refthm{hostProps} shows
  the composed proof will prove it.
  %
  If $P$ was introduced by an extension, \refthm{full-proof-ext} shows
  the composed proof will prove it if the key relation was introduced
  by the same extension.  If the key relation was instead introduced
  by the host language, \refthm{full-proof-host} shows the composed
  proof will prove it.
\end{proof}

